From Relevance to Authority: Authority-aware Generative Retrieval in Web Search Engines

Generative information retrieval (GenIR) formulates the retrieval process as a text-to-text generation task, leveraging the vast knowledge of large language models. However, existing works primarily optimize for relevance while often overlooking document trustworthiness. This is critical in high-stakes domains like healthcare and finance, where relying solely on semantic relevance risks retrieving unreliable information. To address this, we propose an Authority-aware Generative Retriever (AuthGR), the first framework that incorporates authority into GenIR. AuthGR consists of three key components: (i) Multimodal Authority Scoring, which employs a vision-language model to quantify authority from textual and visual cues; (ii) a Three-stage Training Pipeline to progressively instill authority awareness into the retriever; and (iii) a Hybrid Ensemble Pipeline for robust deployment. Offline evaluations demonstrate that AuthGR successfully enhances both authority and accuracy, with our 3B model matching a 14B baseline. Crucially, large-scale online A/B tests and human evaluations conducted on the commercial web search platform confirm significant improvements in real-world user engagement and reliability.

==> Figures_tex/fig_deployment.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{Figures/fig_deployment.png}
% \vspace{-3.5mm}
\caption{Hybrid ensemble pipeline for deploying AuthGR in production search systems.}\label{fig:deployment}
\vspace{-3.5mm}
\end{figure}



==> tables/tab_data_statistics.tex <==
\begin{table}[t]
\centering

\caption{Statistics of the datasets used for each training stage.}
\small
\vspace{-0.5em}
\label{tab:datasets}
\begin{tabularx}{\linewidth}{c c X}
\toprule
\textbf{Stage} & \textbf{\# samples} & \textbf{Description} \\
\midrule
CPT   & 9.85 M & Search-specific corpus from web crawl for domain adaptation. \\
SFT   & 3.95 M & Filtered query–clicked document URL pairs for generative retrieval task. \\
GRPO  & 13.8 K & High-quality queries for policy optimization, using authority scores as rewards. \\
\bottomrule
\end{tabularx}
\vspace{-1.0em}
\end{table}

